'No' Matters: Out-of-Distribution Detection in Multimodality Long Dialogue

Out-of-distribution (OOD) detection in multimodal contexts is essential for identifying deviations in combined inputs from different modalities, particularly in applications like open-domain dialogue systems or real-life dialogue interactions. This paper aims to improve the user experience that involves multi-round long dialogues by efficiently detecting OOD dialogues and images. We introduce a novel scoring framework named Dialogue Image Aligning and Enhancing Framework (DIAEF) that integrates the visual language models with the novel proposed scores that detect OOD in two key scenarios (1) mismatches between the dialogue and image input pair and (2) input pairs with previously unseen labels. Our experimental results, derived from various benchmarks, demonstrate that integrating image and multi-round dialogue OOD detection is more effective with previously unseen labels than using either modality independently. In the presence of mismatched pairs, our proposed score effectively identifies these mismatches and demonstrates strong robustness in long dialogues. This approach enhances domain-aware, adaptive conversational agents and establishes baselines for future studies.

==> Rebuttal.tex <==
General Comment: [This is basically a general response to everyone. We can add this by clicking the "Official Comment" button at the top]

Reviewers, in general, all have contributed valuable suggestions for our paper. Due to the scope of this study, as the first novel study in the multi-round dialogue multi-modality QA, in particular, has relatively limited datasets. Based on the reviewer's comments, we expanded our paper by: (1) adding up our experiments by testing the performance of our score function on other VLM, like BLIP, results[...]; (2)  adding the references suggested by Reviewer Tsq7 and improved our Figure 2. clearer in the text; (3) testing our score function on other dialogue multimodal datasets, including Real MMD and MELD, and the results [....]; (4) adding the theoretical explanation for our proposed score function and gave an analysis based on that under Reviewer S8mJ's comments; (5) testing our score function on BLIP and CLIP for a single utterance dataset, results show that [...], which indicates the significance and necessity of using multi-round dialogue in OOD detection for future multi-modality investigation. More importantly, in real-life applications, it improves the user experience when users encounter multiple questions.    

In our original paper, we have clarified the challenges and barriers of conducting such a study with a multi-round dialogue QA dataset, as no one has ever tried this task in the OOD detection field previously. To give a more practical reduplicate solution for future work, we incorporate the analysis of hyper-parameters in Section 5.4 Line 294-Line 331. Furthermore, we use Natural Language Processing methods combining WordPath distance and semantical similarity in selecting the OOD labels based on language distance since this study emphasises the label from dialogues in OOD detection, so we consider both two aspects from the nature of human languages and provides a linguistics justification based on this selection method. Under comparison with a single modality, our score function demonstrated stable performance in the OOD detection task as shown in Section 5.4.   

We hope this clarifies why we only incorporated limited datasets in the original paper with the practical challenge, despite the reality difficulties, for the added-up experiments, we tried our best to use real-life multi-modal dialogue datasets, and present the performance [...]. We look forward to receiving further feedback on other feasible multi-round QA multi-modality dialogue datasets from the reviewers, and we would be happy to continue working and expanding to test our score function on recommended datasets in the following week before the deadline. 

Notably, Reviewers S8mJ remarked that the presence of adversarial examples designed to fool OOD detection. Instead, this is not the focus of this paper; we aim to analyze the effectiveness and robustness of our proposed OOD detection score function in this new context: Multi-round QA multi-modality datasets with real-life implications. And we appreciate this suggestion, we would love to address this question with adversarial attack attempt in our next work with more focus on security discussion. 

Finally, all the experiments, including the added-up experiments, were conducted on a single NVIDIA RTX 2080 Super GPU, which is easy to reduplicate for future studies in a reasonable time at a relatively low cost.   

=========================
Responses to Reviewer gMAi: [if we click "official comment" inside a review box, we can reply for a reviewer directly]

> Weaknesses: (1). Limited Dataset: Validation is primarily conducted on the VisDial dataset, which may limit the generalizability of the results to other datasets or applications. 

Thanks for bringing this up. As we mentioned in the general comment, the novel area has relatively limited datasets, and most dialogue datasets in NLP are only single modality, or very few multi-modality dialogue datasets mostly for sentiment tasks (don't have labels varieties in images, limited only to happy/sad/neutral these emotions labels and not suitable in OOD detection tasks). But still, we also tested DIAEF on two other datasets, including Real MMD datasets, which have longer dialogue rounds and on MELD (a Multimodal Multi-Party Dataset for Emotion Recognition in Conversation with only single utterance, mainly for sentiment tasks), and the results indicated that [fill here...].  


> Weaknesses: (2). Score Sensitivity: The framework's effectiveness highly depends on the selection of scoring functions and hyperparameters, which might require extensive tuning. 

This is a really good point to address. We addressed this discussion in the original paper in Section 5.4, Line 281-Line 331. 

> Weaknesses: (3). Complexity: The integration of multiple scores and the need for precise alignment between image and dialogue inputs may add to the computational complexity.

All experiments, including the added experiments, were conducted on a single NVIDIA RTX 2080 Super GPU. 

> Questions:
How does the framework perform on datasets with different distributions or types of dialogues and images?

We appreciated for bringing up this valuable point. We intended to discover this point, however, as we pointed out in General Comments, the possible multi-round multi-modality QA datasets are rare and most usually limited in single modality with only dialogue text, which are not suitable in addressing this multi-modality OOD issue. We hope to expand the datasets and compare the different distributions in future research by ourselves. We also tested the proposed score function performance in other datasets, including the Real MMD dataset (in real QA settings with over 40 turns in one dialogue) and MELD (a multimodal multi-party dataset for emotion recognition in conversation with only a single utterance, mainly for sentiment task). Results can be found in responses to Question (2).  

> Limitations (1): Dataset Dependency: The framework’s performance is validated on a specific dataset, and its effectiveness on other datasets is not explored. 

Thanks for bringing this up. As we mentioned in the general comment, the novel area has relatively limited datasets, and most long-dialogue datasets in NLP are only single modality, or very few multi-modality dialogue datasets mostly for sentiment tasks (don't have labels varieties in images, limited only to happy/sad/neutral these emotions labels and not suitable in OOD detection tasks). We also tested DIAEF on two other datasets, including Real MMD datasets, which have longer dialogue rounds and on MELD (a Multimodal Multiparty Dataset for Emotion Recognition in Conversation with only a single utterance, mainly for sentiment tasks), and the results indicated that [fill here...].  

> Limitations (2): Scalability: The computational requirements for training and deploying the framework on large-scale QA systems are not fully addressed. 

This was addressed in the paper in Section 5.3 Line253-254; all experiments were executed on a system featuring a single NVIDIA RTX 2080 Super GPU

> Limitations (3): Generalization: The ability of the framework to generalize to different types of OOD scenarios beyond those tested is not thoroughly examined.

Thanks for raising this point. We discussed three types of OOD (in Figure 1.): mismatched OOD and label OOD pair where the ID label is `cat' and the OOD label is `sport'. The experiments considered the above three OOD conditions. 

==========================
Responses to Reviewer Tsq7 

> Weaknesses:(1) The current work simply applies OOD detection in VQA under dialogue settings. How does the DIAEF framework enhance misalignment detection between images and dialogues compared to single-round QA with images?

Thanks for bringing this up. We aim to target multi-round dialogues since longer QA dialogues provide more contextual information in real-life scenarios instead of single-round QA (usually with limited contextual information in one question and one answer), which are necessary to detect unseen labels when a user is using a QA system to have multi-rounds of interactions for a related picture request. 

> Weaknesses:(2) Limited OOD Type. The framework's applicability in real-world scenarios with no suitable labels and partial mismatches between images and dialogues is unclear. For example, partial mismatches refer to only a few turns of the dialogue mismatched with the image. How does DIAEF address cases above two cases?

We tested DIAEF's performance in the Real MMD dataset, and the results [fill in the results here]. 

> Weaknesses:(3) Performance Under Resource Constraints. Could the authors discuss the framework’s performance and scalability in environments with limited computational resources? It would be beneficial to understand how DIAEF performs under such constraints and whether there are any optimizations that could be applied.

All experiments, including the added experiments, were conducted on a single NVIDIA RTX 2080 Super GPU. 

> Questions: (1). Missing References. The paper omits several relevant references on multi-modal models in OOD scenarios. Consider including the following:

Thank you for this valuable suggestion, and we've added these two references to our paper. 

> Questions: (2) The text in Fig 2 is blurry, making it difficult to read. Also, fig 2 is cluttered with many small sub-figures, making it hard to read and causing confusion. Simplifying the figure or breaking it down into multiple clearer figures would improve readability and effectively convey the information.

We've fixed the issue and made the text clearer in Figure 2.   

> Limitations: (1). The range of models tested is limited. The experiments utilized only the CLIP model, neglecting other models such as BLIP and generative models like LLAVA. Expanding the experiments to include a variety of models would provide a more comprehensive evaluation of the framework's effectiveness.

We've expanded our tests on BLIP, and the results [....]. 

> Limitations: (2). Limited Dataset Diversity. The framework is tested solely on the VisDial dataset, which may limit the generalizability of the results. The dialogues in the VisDial dataset are relatively simple and short, which might not capture the complexity of real-world scenarios. Testing the framework on datasets with more varied and complex dialogues could provide a better understanding of its performance.

We tested DIAEF's performance in the Real MMD dataset, and the results [fill in the results here]. 


=========================
Responses to Reviewer S8mJ:

> Weaknesses (1): Evaluation limited to a single dataset (VisDial).

Thanks for bringing this up. As we mentioned in the general comment, the novel area has relatively limited datasets, and most long-dialogue datasets in NLP are only single modality, or very few multi-modality dialogue datasets mostly for sentiment tasks (don't have labels varieties in images, limited only to happy/sad/neutral these emotions labels and not suitable in OOD detection tasks). We also tested DIAEF on two other datasets, including Real MMD datasets, which have longer dialogue rounds and on MELD (a Multimodal Multiparty Dataset for Emotion Recognition in Conversation with only a single utterance, mainly for sentiment tasks), and the results indicated that [fill here...].  

> Multiplicative combination of alignment and enhancing terms in the DIAEF score seems somewhat ad hoc - no theoretical justification for why this particular combination should work better than alternatives (e.g., additive combination or more complex functions).

[...]

> Weaknesses (2): The selection of OOD labels using semantic distance and WordNet path calculation (Equation 3) may not capture all aspects of distributional shift in real-world scenarios.

We appreciated this point and this is a great point to address.  We intended to discover this point, however, as we pointed out in General Comments, the possible multi-round multi-modality QA datasets are rare and most usually limited in single modality with only dialogue text, which are not suitable in addressing this multi-modality OOD issue. We hope to expand the datasets and compare the different distributions in future research by ourselves. We also tested the proposed score function performance in other datasets, including the Real MMD dataset (in real QA settings) and MELD (a Multimodal Multi-Party Dataset for Emotion Recognition in Conversation with only a single utterance, mainly for sentiment tasks). Results [...].  

> Questions (1): Have you considered evaluating DIAEF on other QA datasets?

See reply to Weakness (1). 

> How does the performance of DIAEF degrade as the dimensionality of the embedding space increases? Is there a theoretical bound on the effectiveness of the cosine similarity measure used in $s(x_I, x_T)$ for high-dimensional spaces?

[...]

> Questions (2): Have you explored the impact of different visual language models beyond CLIP on the performance of DIAEF? How sensitive is the framework to the choice of the embedding model?


> Questions (3): How does DIAEF perform in the presence of adversarial examples designed to fool OOD detection?

This is a great point to consider in future research under this novel direction. Currently, this is not the focus of this paper; we aim to analyze the effectiveness and robustness of our proposed OOD detection score function in this new context: Multi-round QA multi-modality datasets with real-life implications. And we appreciate this suggestion, we would love to address this question with adversarial attack attempts in our next work with more focus on the security discussion. 

> Questions (4): The selection score S(c) in Equation 3 uses equal weights $(w_1 = w_2 = 0.5)$ for semantic and ontological distances. Have you explored learning these weights or using a more sophisticated combination strategy to optimize OOD label selection?

The rationale for designing this method is based on the nature of human language from linguistic theories: Language, in our context, refers to the dialogue label and imagine label, which should consider both the semantic meaning (the contextual meaning of a label's token in dialogue) and ontological distances (how human understand and process a certain token in languages). These two aspects count as equally important in label selection, which has been tested effectively statically (Gan and Jiang, 2013). That's the original design for this score. After receiving your suggestion, we tried other tuning, and the results indicated [....].  

Gan, M., Dou, X., \& Jiang, R. (2013). From ontology to semantic similarity: calculation of ontology‐based semantic similarity. The Scientific World Journal, 2013(1), 793091.

> Limitations: The authors acknowledge some limitations of their work, such as the need for validation on more dialogue-image datasets and the potential for further improvements in score design. 


See responses in Questions (3). 

==========================
Responses to Reviewer Pm2L

> Weakness (1): How does the performance of the VL model itself affect the results of the DIAEF method? Can this influence be demonstrated through experiments? This outcome holds significant reference value for selecting backbone models in practical applications.

Thanks for bringing up this point, and we appreciate this suggestion to improve our study. As we mentioned in the General Comments, we added up the extra experiments with BLIP and with two more datasets. The results indicate [....]. 

> Weakness (2): The WordNet path calculation in L216 is difficult to understand. Could you provide a more detailed explanation or illustrate it with an example?

This is a nice point to address. The rationale for designing this method is based on the nature of human language from linguistic theories that the authors in this study used to develop this function: Language, in our context, the dialogue label and imagine label, should consider both the semantic meaning (the contextual meaning of a label's token in dialogue) and ontological distances (how human understand and process a certain token in languages), these two aspects count equally important in label selection which has been tested effective statically (Gan and Jiang, 2013). That's the original design for this score. For example, when we talk about `Cat', it can refer to an animal or a pet, but it can also refer to a signer named `Doja Cat', which means that a label's real meaning largely depends on context.  

Mathematically, the formula [...]. 

Gan, M., Dou, X., \& Jiang, R. (2013). From ontology to semantic similarity: calculation of ontology‐based semantic similarity. The Scientific World Journal, 2013(1), 793091.
